What is Sentiment Meant to Mean to Language Models?

Sentiment analysis is one of the most widely used techniques in text analysis. Recent advancements with Large Language Models have made it more accurate and accessible than ever, allowing researchers to classify text with only a plain English prompt. However, "sentiment" entails a wide variety of concepts depending on the domain and tools used. It has been used to mean emotion, opinions, market movements, or simply a general ``good-bad'' dimension. This raises a question: What exactly are language models doing when prompted to label documents by sentiment? This paper first overviews how sentiment is defined across different contexts, highlighting that it is a confounded measurement construct in that it entails multiple variables, such as emotional valence and opinion, without disentangling them. I then test three language models across two data sets with prompts requesting sentiment, valence, and stance classification. I find that sentiment labels most strongly correlate with valence labels. I further find that classification improves when researchers more precisely specify their dimension of interest rather than using the less well-defined concept of sentiment. I conclude by encouraging researchers to move beyond "sentiment" when feasible and use a more precise measurement construct.

==> outline.tex <==

Intro
Answer one question, given the poor measurement construct, how do LLMs understand sentiment? 

Literature
- Most definitions of sentiment in the literature define sentiment as some combination of "emotion, opinion, feelings"
    - There people for example say this.
    - This other group defines it as this.
    - This paper still defines it as.
    - These definitions may be fine for Miriam Webster who notes that sentiment does have two meanings, emotion and opinion. But they are unacceptably imprecise as a scientific instrument. 
    - A measurement should not be both. If it is both, what should it do when emotions and opinion conflict? If it is opinion, then which of the many subjects that a document may contain is it an opinon about?
- Sentiment is Opinion
    - market research types generally classified it as opinion. 
    - sentiment analyzer
    - sentiwordnet
- Actually maybe it's emotion?
    - vader
    - LIWC
    - semeval 2017
- Sentiment is when the line goes up or down
    - market headlines dataset

The point is not that any of these tools are necessarily bad (although some are), it's that they can't all be sentiment. These constructs are sometimes highly correlated and more well defined measures may not make a difference. However, they are not necessarily correlated And this can lead to widespread misunderstanding or even a simple lack of clarity about what a particular tool does.

- examples of tools or datasets that do not clarify what they measure.

In cases where sentiment is claiming to measure opinions, is it actually?

What are common sentiment analysis tools measuring?
- LLMs
- LMs
- dictionaries

- Opinion classifiers
- Emotion classifiers
- General "goodness" classifiers

Data
- stance data
- sentiment data

Results
- compare stance
- compare valence
- compare performance across model types

Conclusion and implications.
- In this paper I established that sentiment is a confounded measure. leads to obfuscation of what tools are doing and the misapplication of tools. The same thing can be used to measure sentiment in one application will be used to measure opinion in other.
- Demonstrated that LLMs generally understand sentiment to mean emotional valence. LLMs should not be used as sentiment classifier if opinion is what you are hoping to measure.
- Demonstrated that performance increases by simply asking the model to measure the dimension of interest more precisely.
- Generally speaking, sentiment should be discontinued as a widely used measurement construct. Equating emotions with opinions, market movement, or product reviews is largely an artifact of dictionary based text analysis methods. These assumptions were defensible previously because computational tools that could parse the semantics of a document were not available. This made it impossible to directly infer the opinion or information that a document expressed, and thus assuming a correlation with emotionally laden words or some vague dimension of goodness and badness was the best path forward.
- However, with much more sophisticated language models and classification methods, this assumption is no longer necessary. I thus encourage researchers to be more explicit in defining their dimensions of interest when conducting text analysis.
- In this note I reported performance using generative AI, but such large. sophisticated models are not necessary to disambiguate between dimensions of sentiment. Encoder models like BERT can also be used as supervised classifiers, or zero shot shot classifiers.


